Human-AI Co-design for Clinical Prediction Models

Developing safe, effective, and practically useful clinical prediction models (CPMs) traditionally requires iterative collaboration between clinical experts, data scientists, and informaticists. This process refines the often small but critical details of the model building process, such as which features/patients to include and how clinical categories should be defined. However, this traditional collaboration process is extremely time- and resource-intensive, resulting in only a small fraction of CPMs reaching clinical practice. This challenge intensifies when teams attempt to incorporate unstructured clinical notes, which can contain an enormous number of concepts. To address this challenge, we introduce HACHI, an iterative human-in-the-loop framework that uses AI agents to accelerate the development of fully interpretable CPMs by enabling the exploration of concepts in clinical notes. HACHI alternates between (i) an AI agent rapidly exploring and evaluating candidate concepts in clinical notes and (ii) clinical and domain experts providing feedback to improve the CPM learning process. HACHI defines concepts as simple yes-no questions that are used in linear models, allowing the clinical AI team to transparently review, refine, and validate the CPM learned in each round. In two real-world prediction tasks (acute kidney injury and traumatic brain injury), HACHI outperforms existing approaches, surfaces new clinically relevant concepts not included in commonly-used CPMs, and improves model generalizability across clinical sites and time periods. Furthermore, HACHI reveals the critical role of the clinical AI team, such as directing the AI agent to explore concepts that it had not previously considered, adjusting the granularity of concepts it considers, changing the objective function to better align with the clinical objectives, and identifying issues of data bias and leakage.

==> tabs/aki_perf.tex <==
\begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.7cm}}
\toprule
\textbf{Metric} & \textbf{Kheterpal} & \textbf{Kheterpal} & \textbf{Round 1:} & \textbf{Round 1:} & \textbf{Round 2:}  & \textbf{Round 3:} & \textbf{Zero-shot:} & \textbf{Final?}\\
\textbf{Pre Apr 2024} &\textbf{unweighted}&\textbf{weighted}& \textbf{Outcome-Aware} & \textbf{Outcome-Masked} & \textbf{Clinician Feedback} & \textbf{More precise} & \textbf{openevidence} & \textbf{human annotation?}  \\
\midrule
AUC & 0.646 (0.600,0.694) & 0.681 (0.626,0.729) & 0.803 (0.761,0.843) & 0.805 (0.763,0.844) & 0.808 (0.768,0.845) & 0.795 (0.752,0.836)& 0.766 (0.721, 0.805) & \red{???}\\
% Accuracy &0.490 (0.440,0.540) &N/A& 0.720 (0.677,0.762) & 0.710 (0.662,0.755) & 0.725 (0.682,0.767) &0.713 (0.667,0.755) \\
% Brier Score&N/A&N/A & 0.372 (0.328,0.415) & 0.390 (0.363,0.418) & 0.380 (0.350,0.411) \\
% Log Likelihood& N/A & N/A & -0.553 (-0.606,-0.502) & -0.577 (-0.604,-0.551) & -0.565 (-0.595,-0.531) \\
\toprule
% \end{tabular}
% \begin{tabular}{lp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.7cm}}
% \hline
% \textbf{Metric} & \textbf{Kheterpal} & \textbf{Kheterpal} & \textbf{Round 1:} & \textbf{Round 1:} & \textbf{Round 2:} &  \textbf{Round 3:} & \textbf{Zero-shot:} & \textbf{Final?}\\
\textbf{Apr-Dec 2024?} &\textbf{unweighted}&\textbf{weighted}& \textbf{Outcome-Aware} & \textbf{Outcome-Masked} & \textbf{Clinician Feedback}& \textbf{More precise} & \textbf{openevidence} & \textbf{human annotation?} \\
\midrule
AUC & 0.666 (0.596, 0.733) & 0.728 (0.657, 0.798) &  0.790 (0.722,0.851) & 0.745 (0.678,0.809) & 0.803 (0.738,0.859)  & 0.822 (0.760, 0.879) & 0.801 (0.737, 0.858) & \red{0.8 (0.7,0.9) [placeholder]} \\
% Accuracy & 0.500 (0.430, 0.570) & N/A & 0.675 (0.610, 0.740) & 0.645 (0.575, 0.710) & 0.710 (0.645, 0.775) & 0.755 (0.695, 0.815) & \\
% Brier Score & N/A & N/A & 0.407 (0.348, 0.473) & 0.417 (0.376, 0.460) & 0.396 (0.354, 0.440) & 0.370 (0.324, 0.414) & \\
% Log Likelihood& N/A & N/A & -0.592 (-0.665, -0.516) & -0.604 (-0.652, -0.557) & -0.583 (-0.632, -0.536) & -0.553 (-0.598, -0.508) &\\
\bottomrule
\end{tabular}

==> tabs/aki_prevalences.tex <==
% AKI Stage 2 & 0.06 (0.04, 0.07) \\
% AKI Stage 3 & 0.08 (0.06, 0.10) \\
% AKI Stage 1 & 0.37 (0.33, 0.40) \\
% Male & 0.49 (0.46, 0.53) \\

\begin{tabular}{p{10cm}cc}
\toprule
Concept & Coefficient & Prevalence \\
\midrule
... the surgery being minimally invasive, e.g., laparoscopic or robotic-assisted procedures? & -0.74 & 0.41 (0.37, 0.44) \\
... the patient having hypertension, e.g., high blood pressure or antihypertensive medication use? & 0.31 & 0.54 (0.51, 0.58) \\
... the patient having obesity, e.g., high BMI or overweight status? & 0.39 & 0.32 (0.29, 0.36) \\
... the surgery being urgent or emergent, e.g., requiring immediate attention or intervention? & 0.50 & 0.21 (0.18, 0.23) \\
... the patient having a history of sleep apnea, e.g., witnessed apnea or CPAP use? & 0.51 & 0.20 (0.17, 0.23) \\
... the patient having heart failure, e.g., reduced ejection fraction or history of heart failure exacerbations? & 0.64 & 0.08 (0.06, 0.10) \\
... the patient having an active systemic infection, e.g., sepsis, bacteremia, or requiring therapeutic antibiotics? & 0.72 & 0.07 (0.05, 0.09) \\
... the patient having tachycardia, e.g., heart rate $>$ 100 bpm or palpitations? & 0.88 & 0.16 (0.14, 0.19) \\
... the surgery being major or high-risk, e.g., major abdominal surgery or anticipated blood loss $>$ 500mL? & 0.91 & 0.40 (0.36, 0.43) \\
... the patient having chronic kidney disease, e.g., a history of CKD or elevated creatinine levels? & 1.05 & 0.13 (0.11, 0.16) \\
\bottomrule
\end{tabular}


==> tabs/tbi_perf.tex <==
\begin{tabular}{lcccccc}
\hline
\textbf{Metric} 
& \makecell{\textbf{PECARN}\\\textbf{Baseline}}
& \makecell{\textbf{Round 1}\\Outcome-Aware}
& \makecell{\textbf{Round 1}\\Outcome-Masked}
& \makecell{\textbf{Round 2}\\Clinical\\Feedback}
& \makecell{\textbf{Round 3}\\After Feedback\\+ Filter Leak}
& \makecell{\textbf{Zero-shot}\\Openevidence\\+PECARN} \\
\midrule
AUC 
& 0.697 (0.609, 0.774)
& 0.889 (0.803, 0.962)
& 0.893 (0.808, 0.964)
& 0.869 (0.810, 0.923)
& 0.867 (0.805, 0.921)
& 0.824 (0.753, 0.883) \\
% Accuracy
% & 0.532 (0.485, 0.585)
% & 0.960 (0.938, 0.980)
% & 0.960 (0.938, 0.980)
% & 0.855 (0.800, 0.905)
% & 0.845 (0.800, 0.890)
% & -- \\
% Brier Score
% & --
% & 0.064 (0.038, 0.097)
% & 0.063 (0.040, 0.093)
% & 0.240 (0.177, 0.304)
% & 0.257 (0.193, 0.325)
% & -- \\
% Log Likelihood
% & --
% & -0.126 (-0.172, -0.085)
% & -0.120 (-0.165, -0.080)
% & -0.396 (-0.476, -0.318)
% & -0.422 (-0.509, -0.339)
% & -- \\
\hline
\end{tabular}

==> tabs/tbi_prevalences.tex <==
% \begin{tabular}{ll}
% \toprule
% Concept & Prevalence \\
% \midrule
% ...an occipital hematoma? & 0.04 (0.02, 0.06) \\
% ...a history of concussion? & 0.10 (0.07, 0.13) \\
% ...a frontal headache? & 0.13 (0.10, 0.16) \\
% ...altered mental status? & 0.13 (0.10, 0.16) \\
% ...unconsciousness? & 0.39 (0.34, 0.44) \\
% ...LOC? & 0.39 (0.34, 0.44) \\
% ...a headache? & 0.42 (0.37, 0.47) \\
% ...normal gait? & 0.56 (0.51, 0.61) \\
% ...head trauma? & 0.95 (0.93, 0.97) \\
% ...alert and responsive? & 0.99 (0.97, 1.00) \\
% \bottomrule
% \end{tabular}

% Combined table with concept, coefficient, and prevalence
\begin{tabular}{p{10cm}cc}
\toprule
Concept & Coefficient & Prevalence \\
\midrule
... the patient having normal gait? & -0.22 & 0.56 (0.51, 0.61) \\
... the patient experiencing head trauma? & 0.08 & 0.95 (0.93, 0.97) \\
... the patient experiencing a headache? & 0.25 & 0.42 (0.37, 0.47) \\
... the patient having altered mental status? & 0.73 & 0.13 (0.10, 0.16) \\
... the patient experiencing unconsciousness? & 1.58 & 0.39 (0.34, 0.44) \\
\bottomrule
\end{tabular}
